ZIPA: A family of efficient models for multilingual phone recognition

We present ZIPA, a family of efficient speech models that advances the state-of-the-art performance of crosslinguistic phone recognition. We first curated IPAPack++, a large-scale multilingual speech corpus with 17,132 hours of normalized phone transcriptions and a novel evaluation set capturing unseen languages and sociophonetic variation. With the large-scale training data, ZIPA, including transducer (ZIPA-T) and CTC-based (ZIPA-CR) variants, leverage the efficient Zipformer backbones and outperform existing phone recognition systems with much fewer parameters. Further scaling via noisy student training on 11,000 hours of pseudo-labeled multilingual data yields further improvement. While ZIPA achieves strong performance on benchmarks, error analysis reveals persistent limitations in modeling sociophonetic diversity, underscoring challenges for future research.

==> full_table.tex <==

\begin{longtable}{cccc}
\toprule
Language & Split & Dataset & Total Duration \\ 
\midrule
swa & test & Common Voice & 06:32:48 \\ 
 & & Fleurs & 01:32:41 \\ 
swa & dev & Fleurs & 00:41:31 \\ 
 & & Common Voice & 07:52:16 \\ 
swa & train & Common Voice & 28:48:36 \\ 
 & & Fleurs & 10:06:09 \\ \midrule
spa & dev & Fleurs & 01:10:09 \\ 
 & & Common Voice & 24:02:28 \\ 
 & & Multilingual Librispeech  & 09:59:19 \\ 
spa & test & Common Voice & 24:22:29 \\ 
 & & Fleurs & 02:27:16 \\ 
 & & Multilingual Librispeech & 10:00:13 \\ 
spa & train & Common Voice & 404:00:29 \\ 
 & & Fleurs & 06:43:33 \\ 
 & & Multilingual Librispeech & 917:41:03 \\ \midrule
bel & train & Common Voice & 452:08:22 \\ 
 & & Fleurs & 07:18:15 \\ 
bel & test & Fleurs & 03:06:33 \\ 
 & & Common Voice & 18:58:01 \\ 
bel & dev & Fleurs & 01:21:58 \\ 
 & & Common Voice & 18:51:37 \\ \midrule
tam & test & Fleurs & 01:36:38 \\ 
 & & Common Voice & 12:47:22 \\ 
 & & tamil_shar & 16:48:33 \\ 
tam & train & Common Voice & 76:47:49 \\ 
 & & Fleurs & 06:20:35 \\ 
 & & tamil_shar & 133:17:27 \\ 
tam & dev & Fleurs & 01:02:34 \\ 
 & & Common Voice & 15:31:28 \\ \midrule
kin & dev & Common Voice & 19:46:13 \\ 
kin & train & Common Voice & 1376:18:20 \\ 
kin & test & Common Voice & 18:21:47 \\ \midrule
eng & test & Librispeech & 10:44:42 \\ 
 & & Common Voice & 24:52:23 \\ 
 & & Fleurs & 01:23:15 \\ 
eng & train & Common Voice & 1584:30:15 \\ 
 & & Librispeech & 961:03:15 \\ 
 & & Fleurs & 05:38:28 \\ 
eng & dev & Common Voice & 24:58:10 \\ 
 & & Librispeech & 10:30:32 \\ 
 & & Fleurs & 00:52:38 \\ \midrule
ron & dev & Common Voice & 04:01:58 \\ 
 & & Fleurs & 00:52:44 \\ 
ron & train & Common Voice & 05:44:05 \\ 
 & & Fleurs & 07:38:47 \\ 
ron & test & Common Voice & 04:30:59 \\ 
 & & Fleurs & 01:56:57 \\ \midrule
ell & train & Fleurs & 07:30:24 \\ 
ell & test & Fleurs & 01:28:00 \\ 
ell & dev & Fleurs & 00:38:19 \\ \midrule
jpn & train & Fleurs & 05:03:22 \\ 
 & & Common Voice & 09:22:26 \\ 
jpn & dev & Common Voice & 06:11:07 \\ 
 & & Fleurs & 00:40:00 \\ 
jpn & test & Common Voice & 06:31:55 \\ 
 & & Fleurs & 01:31:15 \\ \midrule
tur & dev & Fleurs & 00:56:35 \\ 
 & & Common Voice & 10:15:45 \\ 
tur & train & Fleurs & 06:25:40 \\ 
 & & Common Voice & 29:30:44 \\ 
tur & test & Fleurs & 02:05:29 \\ 
 & & Common Voice & 12:09:20 \\ \midrule
hun & test & Fleurs & 02:27:11 \\ 
 & & Common Voice & 11:48:38 \\ 
hun & dev & Fleurs & 01:08:06 \\ 
 & & Common Voice & 10:53:25 \\ 
hun & train & Common Voice & 21:15:06 \\ 
 & & Fleurs & 07:00:41 \\ \midrule
mon & dev & Common Voice & 02:35:02 \\ 
 & & Fleurs & 00:58:20 \\ 
mon & train & Fleurs & 08:37:49 \\ 
 & & Common Voice & 03:13:37 \\ 
mon & test & Common Voice & 03:00:56 \\ 
 & & Fleurs & 02:12:25 \\ \midrule
ind & test & Fleurs & 01:53:09 \\ 
 & & Common Voice & 04:09:37 \\ 
ind & dev & Fleurs & 00:58:23 \\ 
 & & Common Voice & 03:49:04 \\ 
ind & train & Common Voice & 07:46:52 \\ 
 & & Fleurs & 06:56:13 \\ \midrule
uig & train & Common Voice & 07:36:34 \\ 
uig & test & Common Voice & 06:15:05 \\ 
uig & dev & Common Voice & 06:10:43 \\ \midrule
ita & train & Common Voice & 83:14:54 \\ 
 & & Fleurs & 06:51:31 \\ 
 & & Multilingual Librispeech & 247:22:40 \\ 
ita & test & Common Voice & 26:23:08 \\ 
 & & Multilingual Librispeech & 05:16:22 \\ 
 & & Fleurs & 02:48:15 \\ 
ita & dev & Fleurs & 01:18:39 \\ 
 & & Multilingual Librispeech & 05:10:32 \\ 
 & & Common Voice & 08:54:18 \\ \midrule
mkd & train & Fleurs & 05:08:08 \\ 
mkd & dev & Fleurs & 01:03:14 \\ 
mkd & test & Fleurs & 02:28:12 \\ \midrule
urd & dev & Common Voice & 03:45:29 \\ 
 & & Fleurs & 00:38:06 \\ 
urd & test & Common Voice & 03:48:41 \\ 
 & & Fleurs & 00:39:34 \\ 
urd & train & Common Voice & 04:58:30 \\ 
 & & Fleurs & 05:20:32 \\ \midrule
vie & test & Common Voice & 00:40:06 \\ 
 & & Fleurs & 02:19:40 \\ 
vie & dev & Fleurs & 01:00:33 \\ 
 & & Common Voice & 00:12:41 \\ 
vie & train & Fleurs & 06:42:36 \\ 
 & & Common Voice & 01:51:31 \\ \midrule
cat & train & Common Voice & 1591:25:03 \\ 
 & & Fleurs & 05:46:13 \\ 
cat & dev & Common Voice & 26:07:11 \\ 
 & & Fleurs & 01:05:25 \\ 
cat & test & Common Voice & 25:36:29 \\ 
 & & Fleurs & 02:25:33 \\ \midrule
fra & train & Common Voice & 661:14:43 \\ 
 & & Multilingual Librispeech & 1076:34:49 \\ 
fra & dev & Common Voice & 19:15:03 \\ 
 & & Multilingual Librispeech & 10:04:16 \\ 
fra & test & Common Voice & 19:14:26 \\ 
 & & Multilingual Librispeech & 10:04:01 \\ \midrule
mya & dev & Fleurs & 01:29:30 \\ 
mya & train & Fleurs & 10:04:25 \\ 
mya & test & Fleurs & 03:14:42 \\ \midrule
kaz & train & kazakh2_shar & 554:47:31 \\ 
 & & kazakh_shar & 318:25:26 \\ 
 & & Fleurs & 08:54:35 \\ 
kaz & test & kazakh_shar & 07:03:56 \\ 
 & & Fleurs & 03:01:16 \\ 
kaz & dev & kazakh_shar & 07:07:44 \\ 
 & & Fleurs & 01:17:22 \\ \midrule
deu & train & Common Voice & 778:17:18 \\ 
 & & Multilingual Librispeech & 1966:30:30 \\ 
 & & Fleurs & 06:52:51 \\ 
deu & test & Common Voice & 22:04:07 \\ 
 & & Fleurs & 02:27:49 \\ 
 & & Multilingual Librispeech & 14:17:34 \\ 
deu & dev & Fleurs & 01:03:34 \\ 
 & & Multilingual Librispeech & 14:16:58 \\ 
 & & Common Voice & 22:20:38 \\ \midrule
kir & dev & Fleurs & 01:06:02 \\ 
kir & test & Fleurs & 02:31:18 \\ 
kir & train & Fleurs & 06:59:30 \\ \midrule
mlt & train & Fleurs & 07:29:59 \\ 
 & & Common Voice & 02:24:53 \\ 
mlt & dev & Fleurs & 01:14:15 \\ 
 & & Common Voice & 02:02:07 \\ 
mlt & test & Fleurs & 02:48:49 \\ 
 & & Common Voice & 02:20:23 \\ \midrule
bos & test & Fleurs & 02:28:14 \\ 
bos & train & Fleurs & 07:34:14 \\ 
bos & dev & Fleurs & 01:05:48 \\ \midrule
srp & train & Common Voice & 01:08:08 \\ 
 & & Fleurs & 08:08:18 \\ 
srp & dev & Fleurs & 00:42:09 \\ 
 & & Common Voice & 00:53:58 \\ 
srp & test & Fleurs & 01:39:41 \\ 
 & & Common Voice & 01:06:39 \\ \midrule
isl & dev & Fleurs & 00:05:58 \\ 
isl & train & Fleurs & 02:06:30 \\ 
isl & test & Fleurs & 00:08:08 \\ \midrule
ori & test & Fleurs & 02:14:44 \\ 
ori & dev & Fleurs & 01:00:05 \\ 
ori & train & Fleurs & 02:25:20 \\ \midrule
pol & test & Common Voice & 11:58:32 \\ 
 & & Multilingual Librispeech & 02:08:38 \\ 
 & & Fleurs & 01:37:33 \\ 
pol & dev & Multilingual Librispeech & 02:04:38 \\ 
 & & Fleurs & 00:43:57 \\ 
 & & Common Voice & 11:44:11 \\ 
pol & train & Fleurs & 07:13:49 \\ 
 & & Multilingual Librispeech & 103:38:57 \\ 
 & & Common Voice & 24:47:44 \\ \midrule
nld & test & Multilingual Librispeech & 12:45:37 \\ 
 & & Fleurs & 00:46:18 \\ 
 & & Common Voice & 14:16:59 \\ 
nld & train & Common Voice & 38:07:31 \\ 
 & & Fleurs & 05:48:46 \\ 
 & & Multilingual Librispeech & 1554:14:38 \\ 
nld & dev & Multilingual Librispeech & 12:45:27 \\ 
 & & Fleurs & 00:22:46 \\ 
 & & Common Voice & 14:11:16 \\ \midrule
slv & train & Fleurs & 05:46:47 \\ 
 & & Common Voice & 01:24:43 \\ 
slv & test & Common Voice & 01:23:20 \\ 
 & & Fleurs & 01:46:55 \\ 
slv & dev & Fleurs & 00:44:31 \\ 
 & & Common Voice & 01:13:29 \\ \midrule
tel & dev & Fleurs & 00:44:46 \\ 
tel & train & Fleurs & 05:52:07 \\ 
tel & test & Fleurs & 01:06:38 \\ \midrule
hin & test & Fleurs & 01:06:50 \\ 
 & & Common Voice & 04:04:19 \\ 
hin & train & Common Voice & 05:17:16 \\ 
 & & Fleurs & 05:08:23 \\ 
hin & dev & Fleurs & 00:37:51 \\ 
 & & Common Voice & 02:56:15 \\ \midrule
ukr & dev & Common Voice & 11:17:03 \\ 
 & & Fleurs & 00:46:37 \\ 
ukr & train & Fleurs & 06:41:46 \\ 
 & & Common Voice & 19:56:08 \\ 
ukr & test & Fleurs & 01:47:01 \\ 
 & & Common Voice & 11:47:21 \\ \midrule
yor & test & Fleurs & 03:15:52 \\ 
 & & Common Voice & 01:05:26 \\ 
yor & dev & Fleurs & 01:33:49 \\ 
 & & Common Voice & 00:47:54 \\ 
yor & train & Common Voice & 01:20:01 \\ 
 & & Fleurs & 08:27:42 \\ \midrule
aze & test & Fleurs & 02:25:26 \\ 
aze & train & Fleurs & 06:53:37 \\ 
aze & dev & Fleurs & 01:06:16 \\ \midrule
zho & dev & Common Voice & 15:49:43 \\ 
zho & test & Common Voice & 17:23:23 \\ 
zho & train & Common Voice & 42:04:06 \\ \midrule
mri & test & Fleurs & 04:31:43 \\ 
mri & dev & Fleurs & 01:51:19 \\ 
mri & train & Fleurs & 13:20:08 \\ \midrule
rus & test & Fleurs & 01:56:15 \\ 
 & & Common Voice & 15:48:22 \\ 
rus & dev & Common Voice & 15:25:36 \\ 
 & & Fleurs & 00:55:25 \\ 
rus & train & Fleurs & 06:16:41 \\ 
 & & Common Voice & 37:26:56 \\ \midrule
swe & dev & Common Voice & 05:40:24 \\ 
swe & test & Common Voice & 06:23:55 \\ 
 & & Fleurs & 01:49:23 \\ 
swe & train & Common Voice & 08:10:51 \\ 
 & & Fleurs & 06:20:35 \\ \midrule
pan & dev & Fleurs & 00:37:34 \\ 
pan & train & Fleurs & 04:57:37 \\ 
pan & test & Fleurs & 01:28:46 \\ \midrule
mar & train & Common Voice & 02:13:16 \\ 
 & & Fleurs & 09:28:59 \\ 
mar & test & Common Voice & 02:34:02 \\ 
 & & Fleurs & 03:02:16 \\ 
mar & dev & Common Voice & 01:39:48 \\ 
 & & Fleurs & 01:13:35 \\ \midrule
dan & test & Common Voice & 02:45:18 \\ 
 & & Fleurs & 02:15:44 \\ 
dan & dev & Fleurs & 00:59:06 \\ 
 & & Common Voice & 02:45:23 \\ 
dan & train & Fleurs & 05:45:06 \\ 
 & & Common Voice & 03:16:57 \\ \midrule
zul & test & Fleurs & 03:02:00 \\ 
zul & train & Fleurs & 11:03:07 \\ 
zul & dev & Fleurs & 01:18:36 \\ \midrule
nob & dev & Fleurs & 00:26:03 \\ 
nob & train & Fleurs & 07:57:37 \\ 
nob & test & Fleurs & 00:55:40 \\ \midrule
por & train & Common Voice & 22:38:41 \\ 
 & & Multilingual Librispeech & 160:57:47 \\ 
 & & Fleurs & 07:45:54 \\ 
por & test & Common Voice & 12:00:02 \\ 
 & & Multilingual Librispeech & 03:44:17 \\ 
 & & Fleurs & 02:29:53 \\ 
por & dev & Common Voice & 11:01:11 \\ 
 & & Fleurs & 01:03:34 \\ \midrule
 & & Multilingual Librispeech & 03:38:39 \\ 
ben & dev & Fleurs & 01:12:40 \\ 
 & & Common Voice & 15:26:32 \\ 
ben & test & Common Voice & 15:49:36 \\ 
 & & Fleurs & 02:45:17 \\ 
ben & train & bengali_shar & 215:24:21 \\ 
 & & Common Voice & 31:49:44 \\ 
 & & Fleurs & 08:10:49 \\ \midrule
bak & dev & Common Voice & 12:26:36 \\ 
bak & train & Common Voice & 139:12:22 \\ 
bak & test & Common Voice & 12:54:48 \\ \midrule
amh & test & Fleurs & 01:16:46 \\ 
amh & dev & Fleurs & 00:34:06 \\ 
amh & train & Fleurs & 08:15:36 \\ \midrule
est & train & Fleurs & 05:22:55 \\ 
 & & Common Voice & 05:49:26 \\ 
est & dev & Fleurs & 01:01:16 \\ 
 & & Common Voice & 04:57:29 \\ 
est & test & Fleurs & 02:22:22 \\ 
 & & Common Voice & 04:55:06 \\ \midrule
cmn & dev & Fleurs & 00:52:17 \\ 
 & & Aishell-1 & 18:04:53 \\ 
cmn & test & Aishell-1 & 10:01:24 \\ 
 & & Fleurs & 02:00:10 \\ 
cmn & train & Aishell-1 & 150:50:14 \\ 
 & & Fleurs & 06:02:12 \\ \midrule
ces & test & Common Voice & 10:21:40 \\ 
 & & Fleurs & 01:54:46 \\ 
ces & train & Fleurs & 06:22:34 \\ 
 & & Common Voice & 22:25:29 \\ 
ces & dev & Fleurs & 00:49:10 \\ 
 & & Common Voice & 10:12:38 \\ \midrule
snd & test & Fleurs & 02:33:14 \\ 
snd & train & Fleurs & 09:08:45 \\ 
snd & dev & Fleurs & 01:06:15 \\ \midrule
glg & dev & Fleurs & 00:53:18 \\ 
 & & Common Voice & 08:22:44 \\ 
glg & test & Fleurs & 02:03:38 \\ 
 & & Common Voice & 09:13:38 \\ 
glg & train & Fleurs & 05:07:12 \\ 
 & & Common Voice & 14:01:47 \\ \midrule
uzb & test & Fleurs & 02:15:12 \\ 
 & & Common Voice & 11:02:25 \\ 
uzb & train & Common Voice & 32:39:44 \\ 
 & & Fleurs & 07:35:51 \\ 
uzb & dev & Common Voice & 09:35:54 \\ 
 & & Fleurs & 00:59:07 \\ \midrule
nya & dev & Fleurs & 01:12:00 \\ 
nya & train & Fleurs & 08:13:52 \\ 
nya & test & Fleurs & 02:45:54 \\ \midrule
tat & dev & Common Voice & 03:20:48 \\ 
tat & test & Common Voice & 05:44:47 \\ 
tat & train & Common Voice & 09:29:35 \\ \midrule
kor & train & Fleurs & 05:40:36 \\ 
kor & test & Fleurs & 01:02:02 \\ 
kor & dev & Fleurs & 00:34:19 \\ \midrule
gle & train & Fleurs & 09:18:51 \\ 
gle & dev & Fleurs & 01:14:28 \\ 
gle & test & Fleurs & 02:45:44 \\ \midrule
eus & test & Common Voice & 10:30:57 \\ 
eus & train & Common Voice & 15:56:07 \\ 
eus & dev & Common Voice & 10:00:15 \\ \midrule
orm & train & Fleurs & 05:06:30 \\ 
orm & dev & Fleurs & 00:03:14 \\ 
orm & test & Fleurs & 00:07:30 \\ \midrule
mal & train & Common Voice & 00:36:24 \\ 
 & & Fleurs & 07:22:11 \\ 
mal & test & Fleurs & 02:51:43 \\ 
 & & Common Voice & 00:13:40 \\ 
mal & dev & Fleurs & 01:21:31 \\ \midrule
ara & test & Fleurs & 01:07:13 \\ 
 & & Common Voice & 12:35:48 \\ 
ara & dev & Common Voice & 12:44:59 \\ 
 & & Fleurs & 00:45:01 \\ 
ara & train & Fleurs & 04:56:05 \\ 
 & & Common Voice & 31:58:14 \\ \midrule
slk & train & Common Voice & 03:26:03 \\ 
 & & Fleurs & 04:32:55 \\ 
slk & test & Fleurs & 02:05:50 \\ 
 & & Common Voice & 03:05:57 \\ 
slk & dev & Fleurs & 00:55:24 \\ 
 & & Common Voice & 02:57:58 \\ \midrule
hau & dev & Common Voice & 00:39:02 \\ 
 & & Fleurs & 01:15:05 \\ 
hau & train & Common Voice & 02:06:03 \\ 
 & & Fleurs & 10:05:18 \\ 
hau & test & Fleurs & 02:28:28 \\ 
 & & Common Voice & 00:50:10 \\ \midrule
yue & dev & Common Voice & 02:52:00 \\ 
yue & test & Common Voice & 03:09:06 \\ 
 & & Fleurs & 02:04:22 \\ 
yue & train & Common Voice & 03:26:30 \\ 
 & & Fleurs & 05:33:36 \\ \midrule
ceb & dev & Fleurs & 00:43:22 \\ 
ceb & test & Fleurs & 01:46:15 \\ 
ceb & train & Fleurs & 09:19:35 \\ \midrule
tha & train & Fleurs & 06:12:42 \\ 
 & & Common Voice & 37:07:21 \\ 
tha & dev & Fleurs & 01:08:14 \\ 
 & & Common Voice & 14:17:19 \\ 
tha & test & Fleurs & 02:33:41 \\ 
 & & Common Voice & 14:59:46 \\ \midrule
ful & test & Fleurs & 02:07:18 \\ 
ful & train & Fleurs & 10:16:26 \\ 
ful & dev & Fleurs & 00:50:37 \\ \midrule
afr & train & Fleurs & 02:42:43 \\ 
afr & dev & Fleurs & 00:29:05 \\ 
afr & test & Fleurs & 00:39:29 \\ \midrule
kat & dev & Common Voice & 04:22:27 \\ 
 & & Fleurs & 00:59:32 \\ 
kat & train & Common Voice & 09:34:08 \\ 
 & & Fleurs & 03:52:10 \\ 
kat & test & Common Voice & 03:40:55 \\ 
 & & Fleurs & 02:22:27 \\ \midrule
fin & test & Fleurs & 02:34:31 \\ 
fin & train & Fleurs & 06:44:46 \\ 
fin & dev & Fleurs & 01:11:05 \\ \midrule
tgk & test & Fleurs & 01:57:38 \\ 
tgk & dev & Fleurs & 00:46:12 \\ 
tgk & train & Fleurs & 06:31:01 \\ \midrule
lit & train & Fleurs & 07:16:38 \\ 
lit & dev & Fleurs & 00:58:19 \\ 
lit & test & Fleurs & 02:18:57 \\ \midrule
sin & train & shinhala_shar & 215:47:11 \\ \midrule
cym & train & Fleurs & 09:07:12 \\ 
cym & dev & Fleurs & 01:29:10 \\ 
cym & test & Fleurs & 03:19:20 \\ \midrule
kmr & test & Common Voice & 04:27:54 \\ 
kmr & dev & Common Voice & 04:13:56 \\ 
kmr & train & Common Voice & 04:55:01 \\ \midrule
msa & test & Fleurs & 01:49:24 \\ 
msa & train & Fleurs & 07:17:01 \\ 
msa & dev & Fleurs & 00:47:17 \\ \midrule
jav & test & Fleurs & 02:13:16 \\ 
jav & train & javanese_shar & 295:46:56 \\ 
 & & Fleurs & 08:36:13 \\ 
jav & dev & Fleurs & 00:56:38 \\ \midrule
xho & test & Fleurs & 02:54:53 \\ 
xho & train & Fleurs & 09:46:42 \\ 
xho & dev & Fleurs & 01:16:16 \\ \midrule
bul & test & Fleurs & 01:26:29 \\ 
bul & train & Fleurs & 07:02:45 \\ 
bul & dev & Fleurs & 00:50:53 \\ \midrule
ina & train & Common Voice & 04:32:09 \\ 
ina & test & Common Voice & 02:07:29 \\ 
ina & dev & Common Voice & 02:35:14 \\ \midrule
skr & dev & Common Voice & 01:14:13 \\ 
skr & train & Common Voice & 01:17:07 \\ 
skr & test & Common Voice & 01:02:44 \\ \midrule
hrv & train & Fleurs & 08:46:37 \\ 
hrv & test & Fleurs & 01:59:04 \\ 
hrv & dev & Fleurs & 00:50:43 \\ \midrule
sna & train & Fleurs & 07:33:33 \\ 
sna & dev & Fleurs & 01:16:13 \\ 
sna & test & Fleurs & 03:01:57 \\ \midrule
som & train & Fleurs & 09:50:14 \\ 
som & test & Fleurs & 03:01:53 \\ 
som & dev & Fleurs & 01:15:45 \\ \midrule
lao & dev & Fleurs & 00:28:05 \\ 
lao & train & Fleurs & 05:34:58 \\ 
lao & test & Fleurs & 01:05:07 \\ \bottomrule
\caption{Detailed statistics of IPAPack++.}
\label{app:plus_stats}
\end{longtable}


==> latex/full_table.tex <==

\begin{longtable}{cccc}
\toprule
Language & Split & Dataset & Total Duration \\ 
\midrule
swa & test & Common Voice & 06:32:48 \\ 
 & & Fleurs & 01:32:41 \\ 
swa & dev & Fleurs & 00:41:31 \\ 
 & & Common Voice & 07:52:16 \\ 
swa & train & Common Voice & 28:48:36 \\ 
 & & Fleurs & 10:06:09 \\ \midrule
spa & dev & Fleurs & 01:10:09 \\ 
 & & Common Voice & 24:02:28 \\ 
 & & Multilingual Librispeech  & 09:59:19 \\ 
spa & test & Common Voice & 24:22:29 \\ 
 & & Fleurs & 02:27:16 \\ 
 & & Multilingual Librispeech & 10:00:13 \\ 
spa & train & Common Voice & 404:00:29 \\ 
 & & Fleurs & 06:43:33 \\ 
 & & Multilingual Librispeech & 917:41:03 \\ \midrule
bel & train & Common Voice & 452:08:22 \\ 
 & & Fleurs & 07:18:15 \\ 
bel & test & Fleurs & 03:06:33 \\ 
 & & Common Voice & 18:58:01 \\ 
bel & dev & Fleurs & 01:21:58 \\ 
 & & Common Voice & 18:51:37 \\ \midrule
tam & test & Fleurs & 01:36:38 \\ 
 & & Common Voice & 12:47:22 \\ 
 & & tamil_shar & 16:48:33 \\ 
tam & train & Common Voice & 76:47:49 \\ 
 & & Fleurs & 06:20:35 \\ 
 & & tamil_shar & 133:17:27 \\ 
tam & dev & Fleurs & 01:02:34 \\ 
 & & Common Voice & 15:31:28 \\ \midrule
kin & dev & Common Voice & 19:46:13 \\ 
kin & train & Common Voice & 1376:18:20 \\ 
kin & test & Common Voice & 18:21:47 \\ \midrule
eng & test & Librispeech & 10:44:42 \\ 
 & & Common Voice & 24:52:23 \\ 
 & & Fleurs & 01:23:15 \\ 
eng & train & Common Voice & 1584:30:15 \\ 
 & & Librispeech & 961:03:15 \\ 
 & & Fleurs & 05:38:28 \\ 
eng & dev & Common Voice & 24:58:10 \\ 
 & & Librispeech & 10:30:32 \\ 
 & & Fleurs & 00:52:38 \\ \midrule
ron & dev & Common Voice & 04:01:58 \\ 
 & & Fleurs & 00:52:44 \\ 
ron & train & Common Voice & 05:44:05 \\ 
 & & Fleurs & 07:38:47 \\ 
ron & test & Common Voice & 04:30:59 \\ 
 & & Fleurs & 01:56:57 \\ \midrule
ell & train & Fleurs & 07:30:24 \\ 
ell & test & Fleurs & 01:28:00 \\ 
ell & dev & Fleurs & 00:38:19 \\ \midrule
jpn & train & Fleurs & 05:03:22 \\ 
 & & Common Voice & 09:22:26 \\ 
jpn & dev & Common Voice & 06:11:07 \\ 
 & & Fleurs & 00:40:00 \\ 
jpn & test & Common Voice & 06:31:55 \\ 
 & & Fleurs & 01:31:15 \\ \midrule
tur & dev & Fleurs & 00:56:35 \\ 
 & & Common Voice & 10:15:45 \\ 
tur & train & Fleurs & 06:25:40 \\ 
 & & Common Voice & 29:30:44 \\ 
tur & test & Fleurs & 02:05:29 \\ 
 & & Common Voice & 12:09:20 \\ \midrule
hun & test & Fleurs & 02:27:11 \\ 
 & & Common Voice & 11:48:38 \\ 
hun & dev & Fleurs & 01:08:06 \\ 
 & & Common Voice & 10:53:25 \\ 
hun & train & Common Voice & 21:15:06 \\ 
 & & Fleurs & 07:00:41 \\ \midrule
mon & dev & Common Voice & 02:35:02 \\ 
 & & Fleurs & 00:58:20 \\ 
mon & train & Fleurs & 08:37:49 \\ 
 & & Common Voice & 03:13:37 \\ 
mon & test & Common Voice & 03:00:56 \\ 
 & & Fleurs & 02:12:25 \\ \midrule
ind & test & Fleurs & 01:53:09 \\ 
 & & Common Voice & 04:09:37 \\ 
ind & dev & Fleurs & 00:58:23 \\ 
 & & Common Voice & 03:49:04 \\ 
ind & train & Common Voice & 07:46:52 \\ 
 & & Fleurs & 06:56:13 \\ \midrule
uig & train & Common Voice & 07:36:34 \\ 
uig & test & Common Voice & 06:15:05 \\ 
uig & dev & Common Voice & 06:10:43 \\ \midrule
ita & train & Common Voice & 83:14:54 \\ 
 & & Fleurs & 06:51:31 \\ 
 & & Multilingual Librispeech & 247:22:40 \\ 
ita & test & Common Voice & 26:23:08 \\ 
 & & Multilingual Librispeech & 05:16:22 \\ 
 & & Fleurs & 02:48:15 \\ 
ita & dev & Fleurs & 01:18:39 \\ 
 & & Multilingual Librispeech & 05:10:32 \\ 
 & & Common Voice & 08:54:18 \\ \midrule
mkd & train & Fleurs & 05:08:08 \\ 
mkd & dev & Fleurs & 01:03:14 \\ 
mkd & test & Fleurs & 02:28:12 \\ \midrule
urd & dev & Common Voice & 03:45:29 \\ 
 & & Fleurs & 00:38:06 \\ 
urd & test & Common Voice & 03:48:41 \\ 
 & & Fleurs & 00:39:34 \\ 
urd & train & Common Voice & 04:58:30 \\ 
 & & Fleurs & 05:20:32 \\ \midrule
vie & test & Common Voice & 00:40:06 \\ 
 & & Fleurs & 02:19:40 \\ 
vie & dev & Fleurs & 01:00:33 \\ 
 & & Common Voice & 00:12:41 \\ 
vie & train & Fleurs & 06:42:36 \\ 
 & & Common Voice & 01:51:31 \\ \midrule
cat & train & Common Voice & 1591:25:03 \\ 
 & & Fleurs & 05:46:13 \\ 
cat & dev & Common Voice & 26:07:11 \\ 
 & & Fleurs & 01:05:25 \\ 
cat & test & Common Voice & 25:36:29 \\ 
 & & Fleurs & 02:25:33 \\ \midrule
fra & train & Common Voice & 661:14:43 \\ 
 & & Multilingual Librispeech & 1076:34:49 \\ 
fra & dev & Common Voice & 19:15:03 \\ 
 & & Multilingual Librispeech & 10:04:16 \\ 
fra & test & Common Voice & 19:14:26 \\ 
 & & Multilingual Librispeech & 10:04:01 \\ \midrule
mya & dev & Fleurs & 01:29:30 \\ 
mya & train & Fleurs & 10:04:25 \\ 
mya & test & Fleurs & 03:14:42 \\ \midrule
kaz & train & kazakh2_shar & 554:47:31 \\ 
 & & kazakh_shar & 318:25:26 \\ 
 & & Fleurs & 08:54:35 \\ 
kaz & test & kazakh_shar & 07:03:56 \\ 
 & & Fleurs & 03:01:16 \\ 
kaz & dev & kazakh_shar & 07:07:44 \\ 
 & & Fleurs & 01:17:22 \\ \midrule
deu & train & Common Voice & 778:17:18 \\ 
 & & Multilingual Librispeech & 1966:30:30 \\ 
 & & Fleurs & 06:52:51 \\ 
deu & test & Common Voice & 22:04:07 \\ 
 & & Fleurs & 02:27:49 \\ 
 & & Multilingual Librispeech & 14:17:34 \\ 
deu & dev & Fleurs & 01:03:34 \\ 
 & & Multilingual Librispeech & 14:16:58 \\ 
 & & Common Voice & 22:20:38 \\ \midrule
kir & dev & Fleurs & 01:06:02 \\ 
kir & test & Fleurs & 02:31:18 \\ 
kir & train & Fleurs & 06:59:30 \\ \midrule
mlt & train & Fleurs & 07:29:59 \\ 
 & & Common Voice & 02:24:53 \\ 
mlt & dev & Fleurs & 01:14:15 \\ 
 & & Common Voice & 02:02:07 \\ 
mlt & test & Fleurs & 02:48:49 \\ 
 & & Common Voice & 02:20:23 \\ \midrule
bos & test & Fleurs & 02:28:14 \\ 
bos & train & Fleurs & 07:34:14 \\ 
bos & dev & Fleurs & 01:05:48 \\ \midrule
srp & train & Common Voice & 01:08:08 \\ 
 & & Fleurs & 08:08:18 \\ 
srp & dev & Fleurs & 00:42:09 \\ 
 & & Common Voice & 00:53:58 \\ 
srp & test & Fleurs & 01:39:41 \\ 
 & & Common Voice & 01:06:39 \\ \midrule
isl & dev & Fleurs & 00:05:58 \\ 
isl & train & Fleurs & 02:06:30 \\ 
isl & test & Fleurs & 00:08:08 \\ \midrule
ori & test & Fleurs & 02:14:44 \\ 
ori & dev & Fleurs & 01:00:05 \\ 
ori & train & Fleurs & 02:25:20 \\ \midrule
pol & test & Common Voice & 11:58:32 \\ 
 & & Multilingual Librispeech & 02:08:38 \\ 
 & & Fleurs & 01:37:33 \\ 
pol & dev & Multilingual Librispeech & 02:04:38 \\ 
 & & Fleurs & 00:43:57 \\ 
 & & Common Voice & 11:44:11 \\ 
pol & train & Fleurs & 07:13:49 \\ 
 & & Multilingual Librispeech & 103:38:57 \\ 
 & & Common Voice & 24:47:44 \\ \midrule
nld & test & Multilingual Librispeech & 12:45:37 \\ 
 & & Fleurs & 00:46:18 \\ 
 & & Common Voice & 14:16:59 \\ 
nld & train & Common Voice & 38:07:31 \\ 
 & & Fleurs & 05:48:46 \\ 
 & & Multilingual Librispeech & 1554:14:38 \\ 
nld & dev & Multilingual Librispeech & 12:45:27 \\ 
 & & Fleurs & 00:22:46 \\ 
 & & Common Voice & 14:11:16 \\ \midrule
slv & train & Fleurs & 05:46:47 \\ 
 & & Common Voice & 01:24:43 \\ 
slv & test & Common Voice & 01:23:20 \\ 
 & & Fleurs & 01:46:55 \\ 
slv & dev & Fleurs & 00:44:31 \\ 
 & & Common Voice & 01:13:29 \\ \midrule
tel & dev & Fleurs & 00:44:46 \\ 
tel & train & Fleurs & 05:52:07 \\ 
tel & test & Fleurs & 01:06:38 \\ \midrule
hin & test & Fleurs & 01:06:50 \\ 
 & & Common Voice & 04:04:19 \\ 
hin & train & Common Voice & 05:17:16 \\ 
 & & Fleurs & 05:08:23 \\ 
hin & dev & Fleurs & 00:37:51 \\ 
 & & Common Voice & 02:56:15 \\ \midrule
ukr & dev & Common Voice & 11:17:03 \\ 
 & & Fleurs & 00:46:37 \\ 
ukr & train & Fleurs & 06:41:46 \\ 
 & & Common Voice & 19:56:08 \\ 
ukr & test & Fleurs & 01:47:01 \\ 
 & & Common Voice & 11:47:21 \\ \midrule
yor & test & Fleurs & 03:15:52 \\ 
 & & Common Voice & 01:05:26 \\ 
yor & dev & Fleurs & 01:33:49 \\ 
 & & Common Voice & 00:47:54 \\ 
yor & train & Common Voice & 01:20:01 \\ 
 & & Fleurs & 08:27:42 \\ \midrule
aze & test & Fleurs & 02:25:26 \\ 
aze & train & Fleurs & 06:53:37 \\ 
aze & dev & Fleurs & 01:06:16 \\ \midrule
zho & dev & Common Voice & 15:49:43 \\ 
zho & test & Common Voice & 17:23:23 \\ 
zho & train & Common Voice & 42:04:06 \\ \midrule
mri & test & Fleurs & 04:31:43 \\ 
mri & dev & Fleurs & 01:51:19 \\ 
mri & train & Fleurs & 13:20:08 \\ \midrule
rus & test & Fleurs & 01:56:15 \\ 
 & & Common Voice & 15:48:22 \\ 
rus & dev & Common Voice & 15:25:36 \\ 
 & & Fleurs & 00:55:25 \\ 
rus & train & Fleurs & 06:16:41 \\ 
 & & Common Voice & 37:26:56 \\ \midrule
swe & dev & Common Voice & 05:40:24 \\ 
swe & test & Common Voice & 06:23:55 \\ 
 & & Fleurs & 01:49:23 \\ 
swe & train & Common Voice & 08:10:51 \\ 
 & & Fleurs & 06:20:35 \\ \midrule
pan & dev & Fleurs & 00:37:34 \\ 
pan & train & Fleurs & 04:57:37 \\ 
pan & test & Fleurs & 01:28:46 \\ \midrule
mar & train & Common Voice & 02:13:16 \\ 
 & & Fleurs & 09:28:59 \\ 
mar & test & Common Voice & 02:34:02 \\ 
 & & Fleurs & 03:02:16 \\ 
mar & dev & Common Voice & 01:39:48 \\ 
 & & Fleurs & 01:13:35 \\ \midrule
dan & test & Common Voice & 02:45:18 \\ 
 & & Fleurs & 02:15:44 \\ 
dan & dev & Fleurs & 00:59:06 \\ 
 & & Common Voice & 02:45:23 \\ 
dan & train & Fleurs & 05:45:06 \\ 
 & & Common Voice & 03:16:57 \\ \midrule
zul & test & Fleurs & 03:02:00 \\ 
zul & train & Fleurs & 11:03:07 \\ 
zul & dev & Fleurs & 01:18:36 \\ \midrule
nob & dev & Fleurs & 00:26:03 \\ 
nob & train & Fleurs & 07:57:37 \\ 
nob & test & Fleurs & 00:55:40 \\ \midrule
por & train & Common Voice & 22:38:41 \\ 
 & & Multilingual Librispeech & 160:57:47 \\ 
 & & Fleurs & 07:45:54 \\ 
por & test & Common Voice & 12:00:02 \\ 
 & & Multilingual Librispeech & 03:44:17 \\ 
 & & Fleurs & 02:29:53 \\ 
por & dev & Common Voice & 11:01:11 \\ 
 & & Fleurs & 01:03:34 \\ \midrule
 & & Multilingual Librispeech & 03:38:39 \\ 
ben & dev & Fleurs & 01:12:40 \\ 
 & & Common Voice & 15:26:32 \\ 
ben & test & Common Voice & 15:49:36 \\ 
 & & Fleurs & 02:45:17 \\ 
ben & train & bengali_shar & 215:24:21 \\ 
 & & Common Voice & 31:49:44 \\ 
 & & Fleurs & 08:10:49 \\ \midrule
bak & dev & Common Voice & 12:26:36 \\ 
bak & train & Common Voice & 139:12:22 \\ 
bak & test & Common Voice & 12:54:48 \\ \midrule
amh & test & Fleurs & 01:16:46 \\ 
amh & dev & Fleurs & 00:34:06 \\ 
amh & train & Fleurs & 08:15:36 \\ \midrule
est & train & Fleurs & 05:22:55 \\ 
 & & Common Voice & 05:49:26 \\ 
est & dev & Fleurs & 01:01:16 \\ 
 & & Common Voice & 04:57:29 \\ 
est & test & Fleurs & 02:22:22 \\ 
 & & Common Voice & 04:55:06 \\ \midrule
cmn & dev & Fleurs & 00:52:17 \\ 
 & & Aishell-1 & 18:04:53 \\ 
cmn & test & Aishell-1 & 10:01:24 \\ 
 & & Fleurs & 02:00:10 \\ 
cmn & train & Aishell-1 & 150:50:14 \\ 
 & & Fleurs & 06:02:12 \\ \midrule
ces & test & Common Voice & 10:21:40 \\ 
 & & Fleurs & 01:54:46 \\ 
ces & train & Fleurs & 06:22:34 \\ 
 & & Common Voice & 22:25:29 \\ 
ces & dev & Fleurs & 00:49:10 \\ 
 & & Common Voice & 10:12:38 \\ \midrule
snd & test & Fleurs & 02:33:14 \\ 
snd & train & Fleurs & 09:08:45 \\ 
snd & dev & Fleurs & 01:06:15 \\ \midrule
glg & dev & Fleurs & 00:53:18 \\ 
 & & Common Voice & 08:22:44 \\ 
glg & test & Fleurs & 02:03:38 \\ 
 & & Common Voice & 09:13:38 \\ 
glg & train & Fleurs & 05:07:12 \\ 
 & & Common Voice & 14:01:47 \\ \midrule
uzb & test & Fleurs & 02:15:12 \\ 
 & & Common Voice & 11:02:25 \\ 
uzb & train & Common Voice & 32:39:44 \\ 
 & & Fleurs & 07:35:51 \\ 
uzb & dev & Common Voice & 09:35:54 \\ 
 & & Fleurs & 00:59:07 \\ \midrule
nya & dev & Fleurs & 01:12:00 \\ 
nya & train & Fleurs & 08:13:52 \\ 
nya & test & Fleurs & 02:45:54 \\ \midrule
tat & dev & Common Voice & 03:20:48 \\ 
tat & test & Common Voice & 05:44:47 \\ 
tat & train & Common Voice & 09:29:35 \\ \midrule
kor & train & Fleurs & 05:40:36 \\ 
kor & test & Fleurs & 01:02:02 \\ 
kor & dev & Fleurs & 00:34:19 \\ \midrule
gle & train & Fleurs & 09:18:51 \\ 
gle & dev & Fleurs & 01:14:28 \\ 
gle & test & Fleurs & 02:45:44 \\ \midrule
eus & test & Common Voice & 10:30:57 \\ 
eus & train & Common Voice & 15:56:07 \\ 
eus & dev & Common Voice & 10:00:15 \\ \midrule
orm & train & Fleurs & 05:06:30 \\ 
orm & dev & Fleurs & 00:03:14 \\ 
orm & test & Fleurs & 00:07:30 \\ \midrule
mal & train & Common Voice & 00:36:24 \\ 
 & & Fleurs & 07:22:11 \\ 
mal & test & Fleurs & 02:51:43 \\ 
 & & Common Voice & 00:13:40 \\ 
mal & dev & Fleurs & 01:21:31 \\ \midrule
ara & test & Fleurs & 01:07:13 \\ 
 & & Common Voice & 12:35:48 \\ 
ara & dev & Common Voice & 12:44:59 \\ 
 & & Fleurs & 00:45:01 \\ 
ara & train & Fleurs & 04:56:05 \\ 
 & & Common Voice & 31:58:14 \\ \midrule
slk & train & Common Voice & 03:26:03 \\ 
 & & Fleurs & 04:32:55 \\ 
slk & test & Fleurs & 02:05:50 \\ 
 & & Common Voice & 03:05:57 \\ 
slk & dev & Fleurs & 00:55:24 \\ 
 & & Common Voice & 02:57:58 \\ \midrule
hau & dev & Common Voice & 00:39:02 \\ 
 & & Fleurs & 01:15:05 \\ 
hau & train & Common Voice & 02:06:03 \\ 
 & & Fleurs & 10:05:18 \\ 
hau & test & Fleurs & 02:28:28 \\ 
 & & Common Voice & 00:50:10 \\ \midrule
yue & dev & Common Voice & 02:52:00 \\ 
yue & test & Common Voice & 03:09:06 \\ 
 & & Fleurs & 02:04:22 \\ 
yue & train & Common Voice & 03:26:30 \\ 
 & & Fleurs & 05:33:36 \\ \midrule
ceb & dev & Fleurs & 00:43:22 \\ 
ceb & test & Fleurs & 01:46:15 \\ 
ceb & train & Fleurs & 09:19:35 \\ \midrule
tha & train & Fleurs & 06:12:42 \\ 
 & & Common Voice & 37:07:21 \\ 
tha & dev & Fleurs & 01:08:14 \\ 
 & & Common Voice & 14:17:19 \\ 
tha & test & Fleurs & 02:33:41 \\ 
 & & Common Voice & 14:59:46 \\ \midrule
ful & test & Fleurs & 02:07:18 \\ 
ful & train & Fleurs & 10:16:26 \\ 
ful & dev & Fleurs & 00:50:37 \\ \midrule
afr & train & Fleurs & 02:42:43 \\ 
afr & dev & Fleurs & 00:29:05 \\ 
afr & test & Fleurs & 00:39:29 \\ \midrule
kat & dev & Common Voice & 04:22:27 \\ 
 & & Fleurs & 00:59:32 \\ 
kat & train & Common Voice & 09:34:08 \\ 
 & & Fleurs & 03:52:10 \\ 
kat & test & Common Voice & 03:40:55 \\ 
 & & Fleurs & 02:22:27 \\ \midrule
fin & test & Fleurs & 02:34:31 \\ 
fin & train & Fleurs & 06:44:46 \\ 
fin & dev & Fleurs & 01:11:05 \\ \midrule
tgk & test & Fleurs & 01:57:38 \\ 
tgk & dev & Fleurs & 00:46:12 \\ 
tgk & train & Fleurs & 06:31:01 \\ \midrule
lit & train & Fleurs & 07:16:38 \\ 
lit & dev & Fleurs & 00:58:19 \\ 
lit & test & Fleurs & 02:18:57 \\ \midrule
sin & train & shinhala_shar & 215:47:11 \\ \midrule
cym & train & Fleurs & 09:07:12 \\ 
cym & dev & Fleurs & 01:29:10 \\ 
cym & test & Fleurs & 03:19:20 \\ \midrule
kmr & test & Common Voice & 04:27:54 \\ 
kmr & dev & Common Voice & 04:13:56 \\ 
kmr & train & Common Voice & 04:55:01 \\ \midrule
msa & test & Fleurs & 01:49:24 \\ 
msa & train & Fleurs & 07:17:01 \\ 
msa & dev & Fleurs & 00:47:17 \\ \midrule
jav & test & Fleurs & 02:13:16 \\ 
jav & train & javanese_shar & 295:46:56 \\ 
 & & Fleurs & 08:36:13 \\ 
jav & dev & Fleurs & 00:56:38 \\ \midrule
xho & test & Fleurs & 02:54:53 \\ 
xho & train & Fleurs & 09:46:42 \\ 
xho & dev & Fleurs & 01:16:16 \\ \midrule
bul & test & Fleurs & 01:26:29 \\ 
bul & train & Fleurs & 07:02:45 \\ 
bul & dev & Fleurs & 00:50:53 \\ \midrule
ina & train & Common Voice & 04:32:09 \\ 
ina & test & Common Voice & 02:07:29 \\ 
ina & dev & Common Voice & 02:35:14 \\ \midrule
skr & dev & Common Voice & 01:14:13 \\ 
skr & train & Common Voice & 01:17:07 \\ 
skr & test & Common Voice & 01:02:44 \\ \midrule
hrv & train & Fleurs & 08:46:37 \\ 
hrv & test & Fleurs & 01:59:04 \\ 
hrv & dev & Fleurs & 00:50:43 \\ \midrule
sna & train & Fleurs & 07:33:33 \\ 
sna & dev & Fleurs & 01:16:13 \\ 
sna & test & Fleurs & 03:01:57 \\ \midrule
som & train & Fleurs & 09:50:14 \\ 
som & test & Fleurs & 03:01:53 \\ 
som & dev & Fleurs & 01:15:45 \\ \midrule
lao & dev & Fleurs & 00:28:05 \\ 
lao & train & Fleurs & 05:34:58 \\ 
lao & test & Fleurs & 01:05:07 \\ \bottomrule
\caption{Detailed statistics of IPAPack++.}
\label{app:plus_stats}
\end{longtable}


==> latex/lang_details.tex <==
\begin{longtable}{cccc}
\toprule
Language & Split & Dataset & Total Duration \\ 
\midrule
swa & train & Common Voice & 28:48:36 \\ 
 & & Fleurs & 10:06:09 \\ \midrule
spa & train & Common Voice & 404:00:29 \\ 
 & & Fleurs & 06:43:33 \\ 
 & & Multilingual Librispeech & 917:41:03 \\ \midrule
bel & train & Common Voice & 452:08:22 \\ 
 & & Fleurs & 07:18:15 \\ \midrule
tam & train & Common Voice & 76:47:49 \\ 
 & & Fleurs & 06:20:35 \\ 
 & & IISc-MILE Tamil ASR Corpus & 133:17:27 \\ \midrule
kin & train & Common Voice & 1376:18:20 \\ \midrule
eng & train & Common Voice & 1584:30:15 \\ 
 & & Librispeech & 961:03:15 \\ 
 & & Fleurs & 05:38:28 \\ \midrule
ron & train & Common Voice & 05:44:05 \\ 
 & & Fleurs & 07:38:47 \\  \midrule
ell & train & Fleurs & 07:30:24 \\  \midrule
jpn & train & Fleurs & 05:03:22 \\ 
 & & Common Voice & 09:22:26 \\  \midrule
tur & train & Fleurs & 06:25:40 \\ 
 & & Common Voice & 29:30:44 \\ \midrule
hun & train & Common Voice & 21:15:06 \\ 
 & & Fleurs & 07:00:41 \\ \midrule
mon & train & Fleurs & 08:37:49 \\ 
 & & Common Voice & 03:13:37 \\ \midrule
ind & train & Common Voice & 07:46:52 \\ 
 & & Fleurs & 06:56:13 \\ \midrule
uig & train & Common Voice & 07:36:34 \\  \midrule
ita & train & Common Voice & 83:14:54 \\ 
 & & Fleurs & 06:51:31 \\ 
 & & Multilingual Librispeech & 247:22:40 \\  \midrule
mkd & train & Fleurs & 05:08:08 \\  \midrule
urd & train & Common Voice & 04:58:30 \\ 
 & & Fleurs & 05:20:32 \\ \midrule
vie & train & Fleurs & 06:42:36 \\ 
 & & Common Voice & 01:51:31 \\ \midrule
cat & train & Common Voice & 1591:25:03 \\ 
 & & Fleurs & 05:46:13 \\  \midrule
fra & train & Common Voice & 661:14:43 \\ 
 & & Multilingual Librispeech & 1076:34:49 \\ \midrule
mya & train & Fleurs & 10:04:25 \\  \midrule
kaz & train & Kazakh Speech Dataset  & 554:47:31 \\ 
 & & Kazakh Speech Corpus & 318:25:26 \\ 
 & & Fleurs & 08:54:35 \\  \midrule
deu & train & Common Voice & 778:17:18 \\ 
 & & Multilingual Librispeech & 1966:30:30 \\ 
 & & Fleurs & 06:52:51 \\  \midrule
kir & train & Fleurs & 06:59:30 \\ \midrule
mlt & train & Fleurs & 07:29:59 \\ 
 & & Common Voice & 02:24:53 \\  \midrule
bos & train & Fleurs & 07:34:14 \\  \midrule
srp & train & Common Voice & 01:08:08 \\ 
 & & Fleurs & 08:08:18 \\  \midrule
isl & train & Fleurs & 02:06:30 \\  \midrule
ori & train & Fleurs & 02:25:20 \\ \midrule
pol & train & Fleurs & 07:13:49 \\ 
 & & Multilingual Librispeech & 103:38:57 \\ 
 & & Common Voice & 24:47:44 \\ \midrule
nld & train & Common Voice & 38:07:31 \\ 
 & & Fleurs & 05:48:46 \\ 
 & & Multilingual Librispeech & 1554:14:38 \\ \midrule
slv & train & Fleurs & 05:46:47 \\ 
 & & Common Voice & 01:24:43 \\ \midrule
tel & train & Fleurs & 05:52:07 \\ \midrule
hin & train & Common Voice & 05:17:16 \\ 
 & & Fleurs & 05:08:23 \\  \midrule
ukr & train & Fleurs & 06:41:46 \\ 
 & & Common Voice & 19:56:08 \\  \midrule 
yor & train & Common Voice & 01:20:01 \\ 
 & & Fleurs & 08:27:42 \\ \midrule
aze & train & Fleurs & 06:53:37 \\  \midrule
zho & train & Common Voice & 42:04:06 \\ \midrule
mri & train & Fleurs & 13:20:08 \\ \midrule
rus & train & Fleurs & 06:16:41 \\ 
 & & Common Voice & 37:26:56 \\ \midrule
swe & train & Common Voice & 08:10:51 \\ 
 & & Fleurs & 06:20:35 \\ \midrule
pan & train & Fleurs & 04:57:37 \\  \midrule
mar & train & Common Voice & 02:13:16 \\ 
 & & Fleurs & 09:28:59 \\ \midrule
dan & train & Fleurs & 05:45:06 \\ 
 & & Common Voice & 03:16:57 \\ \midrule
zul & train & Fleurs & 11:03:07 \\  \midrule
nob & train & Fleurs & 07:57:37 \\  \midrule
por & train & Common Voice & 22:38:41 \\ 
 & & Multilingual Librispeech & 160:57:47 \\ 
 & & Fleurs & 07:45:54 \\ \midrule
ben & train & Crowd-sourced speech for Bengali & 215:24:21 \\ 
 & & Common Voice & 31:49:44 \\ 
 & & Fleurs & 08:10:49 \\ \midrule 
bak & train & Common Voice & 139:12:22 \\  \midrule
amh & train & Fleurs & 08:15:36 \\ \midrule
est & train & Fleurs & 05:22:55 \\ 
 & & Common Voice & 05:49:26 \\ \midrule
cmn & train & Aishell-1 & 150:50:14 \\ 
 & & Fleurs & 06:02:12 \\ \midrule
ces & train & Fleurs & 06:22:34 \\ 
 & & Common Voice & 22:25:29 \\  \midrule
snd & train & Fleurs & 09:08:45 \\ \midrule
glg & train & Fleurs & 05:07:12 \\ 
 & & Common Voice & 14:01:47 \\ \midrule
uzb & train & Common Voice & 32:39:44 \\ 
 & & Fleurs & 07:35:51 \\  \midrule
nya & train & Fleurs & 08:13:52 \\  \midrule
tat & train & Common Voice & 09:29:35 \\ \midrule
kor & train & Fleurs & 05:40:36 \\ \midrule
gle & train & Fleurs & 09:18:51 \\ \midrule
eus & train & Common Voice & 15:56:07 \\  \midrule
orm & train & Fleurs & 05:06:30 \\  \midrule
mal & train & Common Voice & 00:36:24 \\ 
 & & Fleurs & 07:22:11 \\  \midrule
ara & train & Fleurs & 04:56:05 \\ 
 & & Common Voice & 31:58:14 \\ \midrule
slk & train & Common Voice & 03:26:03 \\ 
 & & Fleurs & 04:32:55 \\  \midrule
hau & train & Common Voice & 02:06:03 \\ 
 & & Fleurs & 10:05:18 \\ \midrule
yue & train & Common Voice & 03:26:30 \\ 
 & & Fleurs & 05:33:36 \\ \midrule
ceb & train & Fleurs & 09:19:35 \\ \midrule
tha & train & Fleurs & 06:12:42 \\ 
 & & Common Voice & 37:07:21 \\ \midrule
ful & train & Fleurs & 10:16:26 \\  \midrule
afr & train & Fleurs & 02:42:43 \\  \midrule
kat & train & Common Voice & 09:34:08 \\ 
 & & Fleurs & 03:52:10 \\  \midrule 
fin & train & Fleurs & 06:44:46 \\  \midrule
tgk & train & Fleurs & 06:31:01 \\ \midrule
lit & train & Fleurs & 07:16:38 \\  \midrule
sin & train & Crowd-sourced speech for Sinhala & 215:47:11 \\ \midrule
cym & train & Fleurs & 09:07:12 \\  \midrule
kmr & train & Common Voice & 04:55:01 \\ \midrule
msa & train & Fleurs & 07:17:01 \\  \midrule
jav & train & Crowd-sourced speech for Javanese & 295:46:56 \\ 
 & & Fleurs & 08:36:13 \\  \midrule
xho & train & Fleurs & 09:46:42 \\\midrule
bul & train & Fleurs & 07:02:45 \\ \midrule
ina & train & Common Voice & 04:32:09 \\ \midrule
skr & train & Common Voice & 01:17:07 \\  \midrule
hrv & train & Fleurs & 08:46:37 \\  \midrule
sna & train & Fleurs & 07:33:33 \\  \midrule
som & train & Fleurs & 09:50:14 \\ \midrule
lao & train & Fleurs & 05:34:58 \\ \bottomrule
\caption{Detailed statistics of IPAPack++. Only the train split of the original datasets were kept. Each language is represented by the ISO 639-3 standard code. }
\label{app:plus_stats}
\end{longtable}

